Time-dependent mediators in survival analysis: Modelling direct and indirect effects with the additive hazards model

We discuss causal mediation analyses for survival data and propose a new approach based on the additive hazards model. The emphasis is on a dynamic point of view, that is, understanding how the direct and indirect effects develop over time. Hence, importantly, we allow for a time varying mediator. To define direct and indirect effects in such a longitudinal survival setting we take an interventional approach (Didelez (2018)) where treatment is separated into one aspect affecting the mediator and a different aspect affecting survival. In general, this leads to a version of the non-parametric g-formula (Robins (1986)). In the present paper, we demonstrate that combining the g-formula with the additive hazards model and a sequential linear model for the mediator process results in simple and interpretable expressions for direct and indirect effects in terms of relative survival as well as cumulative hazards. Our results generalise and formalise the method of dynamic path analysis (Fosen et al. (2006), Strohmaier et al. (2015)). An application to data from a clinical trial on blood pressure medication is given.

==> babelbst.tex <==
%%
%% This is file `babelbst.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% merlin.mbs  (with options: `bblbst')
%% 
%% IMPORTANT NOTICE:
%% 
%% For the copyright see the source file.
%% 
%% Any modified versions of this file must be renamed
%% with new filenames distinct from babelbst.tex.
%% 
%% For distribution of the original source see the terms
%% for copying and modification in the file merlin.mbs.
%% 
%% This generated file may be distributed as long as the
%% original source files, as listed above, are part of the
%% same distribution. (The sources need not necessarily be
%% in the same archive or directory.)
%% Copyright 1994-2004 Patrick W Daly
 % ===============================================================
 % IMPORTANT NOTICE:
 % This bibliographic style (bst) file has been generated from one or
 % more master bibliographic style (mbs) files, listed above.
 %
 % This generated file can be redistributed and/or modified under the terms
 % of the LaTeX Project Public License Distributed from CTAN
 % archives in directory macros/latex/base/lppl.txt; either
 % version 1 of the License, or any later version.
 % ===============================================================
 % Name and version information of the main mbs file:
 % \ProvidesFile{merlin.mbs}[2004/02/09 4.13 (PWD, AO, DPC)]
 % This is babelbst.tex for English.
 % It should serve as a model for other languages.
 % Alternatively, store it under a different name (e.g. englbst.tex)
 % and then \input it with a command in babelbst.tex.
\def\bbland{and}                \def\bbletal{et~al.}
\def\bbleditors{Herausgeber}        \def\bbleds{Hg.}
\def\bbleditor{Herausgeber}          \def\bbled{Hg.}
\def\bbledby{herausgegeben von}
\def\bbledition{Auf\/lage}        \def\bbledn{Aufl.}
\def\bblvolume{Band}          \def\bblvol{Bd.}
\def\bblof{von}
\def\bblnumber{Nummer}          \def\bblno{Nr.}
\def\bblin{in}
\def\bblpages{Seiten}            \def\bblpp{S.}
\def\bblpage{Seite}              \def\bblp{S.}
\def\bbleidpp{Seiten}
\def\bblchapter{Kapitel}        \def\bblchap{Kap.}
\def\bbltechreport{Technischer Bericht}
\def\bbltechrep{Techn.\ Ber.}
\def\bblmthesis{Diplomarbeit}
\def\bblphdthesis{Dissertation}
\def\bblfirst{Erste}            \def\bblfirsto{1.}
\def\bblsecond{Zweite}          \def\bblsecondo{2.}
\def\bblthird{Dritte}            \def\bblthirdo{3.}
\def\bblfourth{Vierte}          \def\bblfourtho{4.}
\def\bblfifth{F\^^b{u}nfte}            \def\bblfiftho{5.}
\def\bblst{.}  \def\bblnd{.}  \def\bblrd{.}
\def\bblth{.}
\def\bbljan{Januar}  \def\bblfeb{Februar}  \def\bblmar{M\^^b{a}rz}
\def\bblapr{April}    \def\bblmay{Mai}       \def\bbljun{Juni}
\def\bbljul{Juli}     \def\bblaug{August}    \def\bblsep{September}
\def\bbloct{Oktober}  \def\bblnov{November}  \def\bbldec{Dezember}
\endinput
%%
%% End of file `babelbst.tex'.
